Concerned with Data Contamination? Assessing Countermeasures in Code Language Model

Various techniques have been proposed to leverage the capabilities of code language models (CLMs) for SE tasks. While these techniques typically evaluate their effectiveness using publicly available datasets, the evaluation can be subject to data contamination threats where the evaluation datasets have already been used to train the concerned CLMs. This can significantly affect the reliability of the evaluation. Different countermeasures have been suggested to mitigate the data contamination threat. Countermeasures include using more recent data, curating new data, and refactoring existing data are introduced, yet it is unclear whether these countermeasures could really mitigate data contamination threats to model evaluation. To fill the gap, we systematically study to quantify the impacts of these countermeasures on CLMs' performance. To facilitate the study, we collected over 2 million Python functions with timestamps ranging from January 1st, 2018, to December 31st, 2023. The data created before the models' cut-off date are considered "contaminated data", while the data where the countermeasures are taken are regarded as "cleansed data". We study the impact of these countermeasures by investigating the difference in CLMs' performance on contaminated and cleansed data derived from different countermeasures. Our experiments yield several interesting observations. For instance, CLMs do not necessarily perform worse on data after the models' cut-off date; on the contrary, they sometimes perform better. In addition, refactoring did not always result in decreased performance; it could lead to improvements instead. Furthermore, existing metrics such as perplexity cannot distinguish contaminated/cleansed data. We hope that the results and observations could help deepen the understanding of CLMs' capabilities and inform the community about data contamination.

==> FigureTex/figure-passk.tex <==
\begin{figure*}[ht]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\textwidth]{./Figure/rq-passk.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Pass@K on Code Completion Over Years}
    \label{fig:passk}
\end{figure*} 

==> FigureTex/figure_pass1.tex <==
\begin{figure*}[th]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=0.9\textwidth]{./Figure/rq-full.png}
    \setlength{\abovecaptionskip}{-10pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Overall Comparison on Pass@1 of RQ1-3 
    % \wac{Need to separate if and while. And we don't need to distinguish refactor and new refactor.}
    }
    \label{fig:pass-all}
\end{figure*}

==> FigureTex/ppl_scores_rq23.tex <==
\begin{figure*}[ht]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\textwidth]{./Figure/rq-ppl-score-2.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Scores on Benchmarks and Refactored Code}
    \label{fig:rq-score-2}
\end{figure*} 

==> FigureTex/workflow.tex <==
\begin{figure*}[t]
    \centering
    % \vspace{-0ex}
    \includegraphics[width=1.0\linewidth]{./Figure/workflow.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-0pt}
    \caption{Workflow (Draft)}
    \label{fig:workflow}
\end{figure*} 

==> Tex/051-implementation.tex <==
\framac (Framework for modular analysis of C programs)~\cite{kirchner2015frama,beyer2022static} is an extensible and collaborative platform dedicated to source-code analysis. It is mainly co-developed at the Software Security and Reliability Laboratory of CEA-LIST and the Toccata team of INRIA Saclay.

The \wpplugin plugin in \framac implements deductive verification calculus, a modular sound technique to prove that a property holds after the execution of a function if some other properties hold before it (pre/post condition as seen before).
\wpplugin is able to verify more complex logical annotations and assertions using external automated or interactive provers (mainly AltErgo, Why3 and Coq) but requires extra efforts with the code annotations, including loop annotations. Indeed, to analyze a source code with loops, WP needs a specification for each of them, or it uses an implicit specification, which is equivalent to "anything can happen".

\textbf{Theorem Provers}. The VCs generated by WP can be submitted to an interactive or automatic theorem prover. Frama-C natively supports two provers: the
Alt-Ergo automatic prover and the Coq proof assistant. Other provers are supported through the Why platform1. In the experiments reported in this paper
the following provers were used:
– Alt-ergo 0.95.1
– Z3 4.3.1 (through the Why platform)
